FeatDistill: A Feature Distillation Enhanced Multi-Expert Ensemble Framework for Robust AI-generated Image Detection

The rapid iteration and widespread dissemination of deepfake technology have posed severe challenges to information security, making robust and generalizable detection of AI-generated forged images increasingly important. In this paper, we propose FeatDistill, an AI-generated image detection framework that integrates feature distillation with a multi-expert ensemble, developed for the NTIRE Challenge on Robust AI-Generated Image Detection in the Wild. The framework explicitly targets three practical bottlenecks in real-world forensics: degradation interference, insufficient feature representation, and limited generalization. Concretely, we build a four-backbone Vision Transformer (ViT) ensemble composed of CLIP and SigLIP variants to capture complementary forensic cues. To improve data coverage, we expand the training set and introduce comprehensive degradation modeling, which exposes the detector to diverse quality variations and synthesis artifacts commonly encountered in unconstrained scenarios. We further adopt a two-stage training paradigm: the model is first optimized with a standard binary classification objective, then refined by dense feature-level self-distillation for representation alignment. This design effectively mitigates overfitting and enhances semantic consistency of learned features. At inference time, the final prediction is obtained by averaging the probabilities from four independently trained experts, yielding stable and reliable decisions across unseen generators and complex degradations. Despite the ensemble design, the framework remains efficient, requiring only about 10 GB peak GPU memory. Extensive evaluations in the NTIRE challenge setting demonstrate that FeatDistill achieves strong robustness and generalization under diverse ``in-the-wild'' conditions, offering an effective and practical solution for real-world deepfake image detection.

==> include/macros.tex <==
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\newcommand{\refs}[2]{\hyperref[#1]{\ref*{#1}#2}}

\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}


\providecommand{\difadd}[1]{{\protect\color{black}#1}}

\newtheorem{definition}{Definition}[section]

\makeatletter
\renewcommand{\cvprsect}[1]{%
  % 我们这里手动给 \cvprsection 传入两个“标题版本”：
  % 1. 可选参数 [...]    -> 目录里用的短标题
  % 2. 花括号参数 {...}  -> 正文里显示的长标题

  % 首先给目录用的“短标题”：
  %   这里只放真正的标题 #1，本质上就是你写在 \section{...} 里的文字，
  %   不加 \hskip -1em 也不加那个人工的 "."，
  %   这样目录就不会再往回挤一个点靠在 "A" 上了。
  \cvprsection[#1]%
  % 然后给正文用的“长标题”：
  %   这里保持原cvpr.sty的做法：在标题前注入
  %   \hskip -1em.~ 这段小hack，以便排出 "A. 标题" 这种格式。
  %   \texorpdfstring{TeX里用的}{PDF书签里用的}：
  %   - TeX里用的 = \hskip -1em.~  (用于真正的页面标题)
  %   - PDF书签里用的 = ""         (避免把奇怪的 \hskip 写进书签)
  {\texorpdfstring{\hskip -1em.~}{}#1}%
}
\renewcommand{\cvprsubsect}[1]{%
  \cvprsubsection[#1]%
  {\texorpdfstring{\hskip -1em.~}{}#1}%
}
\makeatother

\newcommand{\reviewerheader}[1]{%
  \vspace{-1.25mm}
  \noindent\rule{\linewidth}{1pt}\par
  \vspace{-0.75mm}
  \noindent\textbf{#1}\par
  \vspace{-2.5mm}
  \noindent\rule{\linewidth}{0.5pt}\par
  % \vspace{-0.25mm}
}

\newcommand{\alg}{\texttt{FeatDistill}\xspace}
